Secure Hypersphere Range Query on Encrypted Data

Spatial queries like range queries, nearest neighbor, circular range queries etc. are the most widely used queries in the location-based applications. Building secure and efficient solutions for these queries in the cloud computing framework is critical and has been an area of active research. This paper focuses on the problem of Secure Circular Range Queries (SCRQ), where client submits an encrypted query (consisting of a center point and radius of the circle) and the cloud (storing encrypted data points) has to return the points lying inside the circle. The existing solutions for this problem suffer from various disadvantages such as high processing time which is proportional to square of the query radius, query generation phase which is directly proportional to the number of points covered by the query etc. This paper presents solution for the above problem which is much more efficient than the existing solutions. Three protocols are proposed with varying characteristics. It is shown that all the three protocols are secure. The proposed protocols can be extended to multiple dimensions and thus are able to handle Secure Hypersphere Range Queries (SHRQ) as well. Internally the proposed protocols use pairing-based cryptography and a concept of lookup table. To enable the efficient use of limited size lookup table, a new storage scheme is presented. The proposed storage scheme enables the protocols to handle query with much larger radius values. Using the SHRQ protocols, we also propose a mechanism to answer the Secure range Queries. Extensive performance evaluation has been done to evaluate the efficiency of the proposed protocols

==> Application.tex <==

\section{Solution Applications}
The presented SHRQ solution  can be used to build secure solutions around following queries:
\begin{enumerate}[a.]
	\item Range Queries: Range queries over a column can be of two types:
	\begin{enumerate}[i.]
		\item Close Range : These queries involve selection of values between close range $[Q_L,Q_R]$ like $Q_L < Col <Q_R$.
		\item Open Range: These queries involve selection of values w.r.t. open range $[Q_L,\infty)$ or $(-\infty,Q_R,]$  like $Q_L < Col$ or $Col < Q_R$. Given the statistical information of Max, Min w.r.t. each column the Open range queries can be converted to close range queries like $Q_L < Col \equiv Q_L < Col < Col_{Max}$ and $Col < Q_R \equiv Q_{Min} < Col < Q_R$
	\end{enumerate}
It can be observed that SHRQ w.r.t. single dimension $(d=1)$ becomes a range query.

	Given any range query of form $[Q_L,Q_R]$ w.r.t. $Col$ $i$, it can be converted to  SHRQ query with center $q_i=(Q_L+Q_R)/2$ and  Radius $R=(Q_R-Q_L)/2$.  To incorporate the support for range queries Data Component and Query Component is required to be modified as following:
	\begin{enumerate}
			\item Data Component : $\{m_1,\cdots,m_n,1,||m_1||^2\cdots,||m_n||^2\}$
		\item Query Component (w.r.t. $i^{th} Col$) : $\{0_1,\cdots,0_{i-1}, 2q_i,0_{i+1}\\\cdots,0_n,R^2-||q_i||^2,0_1,\cdots,0_{i-1},-1_i,0_{i+1}\cdots,0_n\}$
	\end{enumerate}
	\item Circular Range Queries (CRQ): CRQ solution is the direct application of the SHRQ. The SHRQ solution w.r.t. 2 dimensional data is solution to CRQ. Unlike  \cite{CRQ1,CRQ2} where the query generation time is proportional to the solution space, in SHRQ query phase just involve the center point and radius as input to get the encrypted query component. The CRQ query w.r.t. large radius can be handled in the similar way by considering the big circle as set of circular disks and the data points are evaluated by using CheckIfInside function in the varying euclidean spaces. 
	\item Minimum Bounded Rectangle (MBR): Any polygon or polyhedron can be converted to simple MBR by computing minimum and maximum reach of the respective shape in each dimension. The solution of MBR query consists of solving range queries w.r.t. each dimension of MBR. The data component which satisfies all the range queries is returned as solution of the MBR region. Queries w.r.t. random shape polygon/polyhedrons can be answered using the MBR queries. However such queries will require a second stage filtration on the result points by the client to check if the point is lying inside the polygon.  
\end{enumerate}

==> SHRQ.tex <==

\section{Secure HypherSphere Range Query}
In this section we first present a SHRQ solution using BGN encryption scheme. Thereafter we show the drawbacks of the solutions and then propose the Data hidden (DH SHRQ) scheme. The Data Component and Query Component representation are same as defined earlier in section ?. These representations will be used during the TupleEncryption and QueryEncryption procedures of the schemes.
\subsection{SHRQ using BGN}
The SHRQ protocols defined under this scheme are as follow:
\begin{itemize}
	\item KeyGen: Key Generation procedure invokes the KeyGen function of BGN Cryptosystem which generates the key parameters $\{q_1,q_2,\mathbb{G,G}_T,e,g,h,N\}$. Since the solution is going to be hosted on the cloud, only computationally required information is shared with cloud. Thus $\{\mathbb{G,G}_T,e,N\}$ is shared with the cloud. As is explained in QueryEncryption, $q_1$ is also shared with cloud for decision computation. The other key parameters $\{q_2,g,h\}$ are kept as private as used in encryption procedures.
	\item TupleEncryption: This function is called by DO to encrypt the data component. Each parameter of the vector is encrypted using the encryption function of BGN cryptosystem. 
	$C_i = g^{m_i}h^r$. Let $m'$ represents the encrypted data component.
		\item Query Encryption: This function is called by DO to encrypt Query component and provide the look up table hash that is used by CS during CheckIfInside  procedure. DO choses two random elements $\alpha, \beta \in \mathbb{Z}_N$ and encrypts the Query Component as below:
		\begin{equation*}
			q' =
			\begin{cases}
				g^{(q_i + \beta)\alpha}h^r & \text{if }i=n+1\\
				g^{q_i \alpha}h^r&\text{otherwise}\\
			\end{cases}
		\end{equation*}
		Lookup table $\mathcal{L}$ is prepared by DO as following:
			\begin{equation*}
		\mathcal{L} = \{g^{(x+\beta)\alpha q_1} \text{, where }x\in[0,|\mathcal{L}|]\\\}
		\end{equation*}
		$|\mathcal{L}|$ represents the size of look up table. The length of the lookup table should be more than the $R^2$. To reduce space of $\mathcal{L}$, DO creates set of hash values of values in $\mathcal{L}$ represented by $\mathcal{H\{L\}}$ using hash function instance $\mathcal{H}$.
		
		Collectively $\{q', \mathcal{H\{L\}},\mathcal{H}\}$ represent the encrypted query which is sent to CS.
	\item CheckIfInside: This procedure is called by CS to make the decision on encrypted data point stored at cloud. The input of the procedure is the encrypted data component $m'$ and the encrypted query $\{q', \mathcal{H\{L\}},\mathcal{H}\}$ and the output is  boolean flag True/False representing if the Data lies inside hyper-sphere or not. The steps involved in the procedure are as follow:
	\begin{enumerate}[a.]
		\item Dot product between $m'$ and $q'$:  This is computed using the homomorphic properties of BGN which involves $(n+2)$ pairwise bilinear operation of respective components of $m',q'$ and then modular multiplication operations of the $n+2$ values in $\mathbb{G}_T$ group.
		\item Flag Decision : The value thus computed is of form $g^lh^r \in \mathcal{G}_T$. First CS removes the randomization $h^r$  by computing the modular exponentiation  w.r.t. $q_1$. Then it  checks for the presence of $\mathcal{H}\{g^l\}$ in $\mathcal{H\{L\}}$. If value exists then return True or else return False.
	\end{enumerate}
\end{itemize}
It can be observed that though the encryption elements $g,h$ of $\mathcal{PK}$ of BGN are kept secret, the key $\mathcal{SK}:q_1$ is revealed to CS, which is  used for de randomization in procedure  CheckIfInside. The immediate drawback arising due CS knowing $q_1$ is that each attribute of  data  
components can be de randomized, thus revealing the frequency information of each attribute.

Secondly the solution presented will not  work for the queries with large values of $R$, as the size of Hash value set $\mathcal{H\{L\}}$ is required to be more than $R$.

Apart from the presented solution of BGN, another approach of using secure H/W or proxy server can also be used. The de randomization in Flag Decision can be done in secure H/W and thus securing the data. But the solution will too be limited to smaller range radius queries. And also the presence of extra H/W adds up the cost of cloud client.

\subsection{Secure Data SHRQ}
 Following we present our proposed SHRQ solution. The solution will handle the following two shortcomings of SHRQ using BGN :
 \begin{enumerate}
 	\item Data Frequency Hiding SHRQ : No essential parameter like $q_1$ is shared with cloud. Thus securing data against frequency leakage.
 	\item Handling Large values of $R$: We present a storage mechanism that can be used to handle queries with large values of $R$.
 \end{enumerate}

\subsubsection{Frequency Hiding SHRQ}
The SHRQ protocols involved under this scheme are as follows:
\begin{itemize}
	\item KeyGen : Call the group generating algorithm with security parameter $1^\lambda$ which generates the parameters $\{q_1,q_2,\mathbb{G,G}_T,e\}$. Here, $q_1,q_2$ are prime numbers and $N=q_1q_2$ is the order of composite groups $\mathbb{G,G}_T$. For encryption further we generate following parameters :
\begin{enumerate}[a.]
	\item Since $ \mathbb{G} $ is composite order of $q_1\times q_2$, it will contain two subgroups $\mathbb{R,S}$ of order $q_1, q_2$. Generate two random generators $\mathbf{r,s}$ from subgroups $\mathbb{R,S}$ respectively.
	\item Generate two $n+2$ size random vectors $A,B$ s.t. dot product, $A.B^T = \text{\LARGE\calligra{r}}.q_1$. Here,{ \LARGE\calligra r} is a random integer in $Z_N$. 
\end{enumerate}
Parameters $\{N,\mathbb{G,G}_T,e\}$ are shared with cloud and all other information is kept secret.
\item TupleEncryption : Select a random integer$\text{ \LARGE\calligra r}_m \in Z_N$. And encrypt each attribute of the data component as:
\begin{equation*}
m' =r^{m_i}s^{\text{\large\calligra r}_mA_i} \text{   } i \in [0,n+2]
\end{equation*}
\item QueryEncryption : This procedure generates encryption of query component and a look table hash. DO choses three random integers $\alpha,\beta, \text{\LARGE\calligra r}_q \in Z_N$ and encrypts the Query Component as below:
\begin{equation*}
q' =
\begin{cases}
r^{(q_i + \beta)\alpha}s^{\text{\large\calligra r}_qB_i} & \text{if }i=n+1\\
r^{q_i \alpha}s^{\text{\large\calligra r}_qB_i}&\text{otherwise}\\
\end{cases}
\end{equation*}
Lookup table hash $\mathcal{H\{L\}}$ is prepared in similar way like before :
\begin{equation*}
\mathcal{L} = \{g^{(x+\beta)\alpha q_1} \text{, where }x\in[0,|\mathcal{L}|]\\\}
\end{equation*}
$|\mathcal{L}|$ represents the size of look up table. DO creates set of hash values of values in $\mathcal{L}$ represented by $\mathcal{H\{L\}}$ using hash function instance $\mathcal{H}$. $\{q', \mathcal{H\{L\}},\mathcal{H}\}$ represent the encrypted query which is sent to CS.
\item CheckIfInside : The procedure involves steps of calculation of dot product between encrypted  $m',q'$ and using it then making the flag decision True/False of whether the point lies inside hyper-sphere or not. The input to the procedure is $m',\{q', \mathcal{H\{L\}},\mathcal{H}\}$. The steps are explained as follows:
\begin{enumerate}[a.]
\item 	Dot product between $m'$ and $q'$: First, for each attribute in $m'$ and $q'$ a bilinear mapping is computed among the respected pairs as follow:
\begin{align*}
e(m'_i,q'_i) =
\begin{cases}
e(r^{m_i}s^{\text{\large\calligra r}_mA_i},r^{(q_i + \beta)\alpha}s^{\text{\large\calligra r}_qB_i}) & \text{if }i=n+1\\
e(r^{m_i}s^{\text{\large\calligra r}_mA_i},r^{q_i \alpha}s^{\text{\large\calligra r}_qB_i})&\text{otherwise}\\
\end{cases}
\\=
\begin{cases}
e(r,r)^{m_i(q_i + \beta)\alpha}e(s,s)^{\text{\large\calligra r}_m\text{\large\calligra r}_qA_iB_i}) & \text{if }i=n+1\\
e(r,r)^{m_iq_i \alpha}e(s,s)^{\text{\large\calligra r}_m\text{\large\calligra r}_qA_iB_i})&\text{otherwise}\\
\end{cases}
\end{align*}
Now, compute the modular multiplication operations in group $\mathbb{G}_T$ of $n+2$ values. The value $T$ thus computed will be:
\begin{align*}
T &= e(r,r)^{(m.q+\beta)\alpha}e(s,s)^{\text{\large\calligra r}_m\text{\large\calligra r}_qAB}\\
&= e(r,r)^{(m.q+\beta)\alpha}&\text{as } e(s,s)^{\text{\large\calligra r}_m\text{\large\calligra r}_qAB}=1
\end{align*}
\item Flag Decision: Check for the presence of $\mathcal{H}\{T\}$ in $\mathcal{H\{L\}}$. If value exists then return True, else return False.
\end{enumerate}
\end{itemize}
The shortcoming of data frequency leakage in SHRQ using BGN is handled in the proposed scheme as CS will not be able to remove the randomness of $\text{\LARGE\calligra r}_m,\text{\LARGE\calligra r}_q$ from the data component and query component. 

Following we present the storage mechanism that can be used by DO w.r.t. data component, so that the Frequency Hiding SHRQ scheme can be used to answer queries for large values of $R$.

\subsubsection{Coarse grained Granular Storage}
